Detecting Activations over Graphs using Spanning Tree Wavelet Bases

We consider the detection of activations over graphs under Gaussian noise, where signals are piece-wise constant over the graph. Despite the wide applicability of such a detection algorithm, there has been little success in the development of computationally feasible methods with proveable theoretical guarantees for general graph topologies. We cast this as a hypothesis testing problem, and first provide a universal necessary condition for asymptotic distinguishability of the null and alternative hypotheses. We then introduce the spanning tree wavelet basis over graphs, a localized basis that reflects the topology of the graph, and prove that for any spanning tree, this approach can distinguish null from alternative in a low signal-to-noise regime. Lastly, we improve on this result and show that using the uniform spanning tree in the basis construction yields a randomized test with stronger theoretical guarantees that in many cases matches our necessary conditions. Specifically, we obtain near-optimal performance in edge transitive graphs, $k$-nearest neighbor graphs, and $\epsilon$-graphs.

==> UST_back.tex <==
\section{Uniform Spanning Tree Basis}



\subsection{Constructing USTs}

In stage (3) of the detection framework, we were given the opportunity to evaluate our test according to some fixed random algorithm.
We will now examine the performance of the spanning tree wavelet detector, when the spanning tree is drawn according to a UST.
First, we will explore the construction of the UST and examine key properties.

Aldous-Broder, sampling probability.

\begin{lemma}
In expectation, the cut size of a fixed signal $x \in \{0,1\}^V$ within the tree relative to that in the graph is proportionate to the average effective resistance of the induced cut.
Denote by $C \in E$ the cut induced by $x$.
\[
\frac{\EE_\tau |\tau \cap C|}{\|\xb\|_0} = \frac{1}{\| \xb \|_0} \sum_{e \in C} r_e \le \frac{1}{\| \xb \|_0} \sum_{e \in C} \frac{1}{k_e}
\]
where $k_e$ is the edge connectivity of $e$.
For a graph with degree bounded by $d$ we have the inequality,
\[
\EE_\tau |\tau \cap C| \ge \frac{|C|}{d}
\]
Furthermore, for an unweighted graph,
\[
\EE_\tau |\tau \cap C| \le |C|
\]
by Raleigh's monotonicity principle.
\end{lemma}

Hence, we can expect that for a given cut in the graph, that the cut size in the tree will look like the effective resistance (which bounds the edge connectivity).
Moreover we cannot expect an improvement over a factor of $1/d$.
This coincides with the example when the cut consists of a single edge, then the edge connectivity is $1$, while the spanning tree necessarily passes though this edge and the LHS is 1.
The simplest algorithms for graph sparsifiers are based on Thompson sampling edges based on their connectivity or conductance.
This facilitates a simple analysis because the independence of the sampling allows us to use basic Chernoff bounds to control the deviation of $\delta_\tau(A)$ from its expectation.
Clearly the UST does not independently sample edges, but it does have the well documented property of negative association, that the inclusion of an edge decreases the probability that another edge is included.
The following lemma states a concentration result for the UST, based on negative association.

\begin{lemma}
For a fixed induced cut $C \subset E$, 
\[
\PP_\tau \{ \frac{|\tau \cap C|}{|C|} \ge (1 + \delta) \frac{1}{|C|} \sum_{e \in C} r_e \} \le \left( \frac{e^\delta}{(1 + \delta)^{1 + \delta}} \right)^{\sum_{e \in C} r_e} 
\]
\end{lemma}

Let $R$ be the minimum effective resistance of the cuts in your class $\Ccal$, namely $R = \min_{C \in \Ccal} \sum_{e \in C} r_e$.
We have the following probabilistic bound on the overlap between the UST and the cut $C \in \Ccal$,
\begin{theorem}
  \label{thm:USTbdd}

  Fix $C \in \Ccal$.
  Draw $\tau \sim \textrm{ UST}(G)$ then with probability at least $1 - \gamma$,
\[
\frac{|\tau \cap C|}{|C|} \le \frac{1}{|C|} \left(R + \sqrt{2 R} + \frac{1}{3} \log(1/\gamma) \right)
\]

\end{theorem}
 
Now that we have a concentration result for a fixed cut $C$, it is customary to bound the size of the class of cuts that we are considering.
A particularly impressive approach is the construction of an edge contraction algorithm, that reconstructs any cut with probability that can be bounded from above.
This allows one to bound the number of such cuts from above by the reciprocal of this probability.

\begin{lemma}
Some things.
\end{lemma} 

\begin{proof}

Consider the random variable $\xb$ drawn uniformly from the hypercube $H_n = \{-1,1\}^n$.
We are interested in bounding the probability that $\xb$ falls within the ellipsoid $E(\Lb) = \{ \xb \in H_n: \xb^\top \Lb \xb \le \rho \}$.
This is clearly equivalent to bounding the size of $E(\Lb)$.
Notice that $\EE \xb = 0$ and $\xb \overset{d}{=} -\xb$.
Consider the spectral decomposition guaranteed by Mercers theorem for $\Lb$: 
\[
\xb^\top \Lb \xb = \sum_{i = 1}^n \lambda_i ( \ub_i^\top \xb )^2
\]
Now let $\mu_i$ be the median of $( \ub_i^\top \xb )^2$.
\begin{claim}
$\mu_i \le \mu$ for constant $\mu$ for all $n$. 
\end{claim}

\begin{proof}
We can use Bernstein's but I have a feeling that we can show that the median is less than the mean which is $1$.
\end{proof}

Let $y_i = \mu_i I\{ ( \ub_i^\top \xb )^2 > \mu_i \}$ then define the variable $g(\xb) = \sum_i \lambda_i y_i$.
Because $y_i \le ( \ub_i^\top \xb )^2$ we have the bound $g(\xb) \le \xb^\top \Lb \xb$.
Thus, $\PP \{ g(\xb) \le rho \} \ge \PP \{ \xb \in E \}$.
Note that $\EE y_i = \frac{\mu_i}{2}$, but that $y_i$ are not independent.  
Amazingly, $y_i$ enjoy the negative association property, and hence satisfy the bound,
\[
\PP \{ \sum_{i=1}^n a_i (\frac{y_i}{\mu_i}) \le (1 - \delta) \frac{\sum_{i=1}^n a_i }{2} \} \le e^{-\delta ^2 (\sum a_i) / 4}
\]
with $a_i = \frac{\lambda_i \mu_i}{\lambda_n \mu}$.
Hence,
\[
\PP \{ \sum_i \lambda_i y_i \le \frac{(1 - \delta)}{2} \sum_i \lambda_i \mu_i \} \le e^{-\delta ^2 (\sum a_i) / 4}
\]


\end{proof}



